Antineutrino Energy Spectrum Unfolding Based on the Daya Bay Measurement and Its Applications

The prediction of reactor antineutrino spectra will play a crucial role as reactor experiments enter the precision era. The positron energy spectrum of 3.5 million antineutrino inverse beta decay reactions observed by the Daya Bay experiment, in combination with the fission rates of fissile isotopes in the reactor, is used to extract the positron energy spectra resulting from the fission of specific isotopes. This information can be used to produce a precise, data-based prediction of the antineutrino energy spectrum in other reactor antineutrino experiments with different fission fractions than Daya Bay. The positron energy spectra are unfolded to obtain the antineutrino energy spectra by removing the contribution from detector response with the Wiener-SVD unfolding method. Consistent results are obtained with other unfolding methods. A technique to construct a data-based prediction of the reactor antineutrino energy spectrum is proposed and investigated. Given the reactor fission fractions, the technique can predict the energy spectrum to a 2% precision. In addition, we illustrate how to perform a rigorous comparison between the unfolded antineutrino spectrum and a theoretical model prediction that avoids the input model bias of the unfolding method.

==> Antineutrino Energy Spectrum Unfolding Based on the Daya Bay Measurement and Its Application/CPC.tex <==
%%% Generation information for this file
%%% Tue Dec 22 10:59:39 2020
%%% /Users/djaffe/Documents/Reactor/work/trunk/NuWa-trunk/dybgaudi/Documentation/AuthorList/2021_Anue_Unfold
%%% ../AuthGen.py dyb_collabotion_list_20200401.xls 20200401 -1 TRUE 
\newcommand{\ECUST}{1}
\newcommand{\Wisconsin}{2}
\newcommand{\BNL}{3}
\newcommand{\NTU}{4}
\newcommand{\IHEP}{5}
\newcommand{\NUU}{6}
\newcommand{\TsingHua}{7}
\newcommand{\SZU}{8}
\newcommand{\ZSU}{9}
\newcommand{\NCEPU}{10}
\newcommand{\CUHK}{11}
\newcommand{\Siena}{12}
\newcommand{\UCI}{13}
\newcommand{\USTC}{14}
\newcommand{\Charles}{15}
\newcommand{\Dubna}{16}
\newcommand{\UIUC}{17}
\newcommand{\LBNL}{18}
\newcommand{\IIT}{19}
\newcommand{\BNU}{20}
\newcommand{\XJTU}{21}
\newcommand{\Yale}{22}
\newcommand{\CIAE}{23}
\newcommand{\SDU}{24}
\newcommand{\GXU}{25}
\newcommand{\VirginiaTech}{26}
\newcommand{\NCTU}{27}
\newcommand{\UC}{28}
\newcommand{\TempleUniversity}{29}
\newcommand{\DGUT}{30}
\newcommand{\UCB}{31}
\newcommand{\HKU}{32}
\newcommand{\NanKai}{33}
\newcommand{\SJTU}{34}
\newcommand{\Princeton}{35}
\newcommand{\CalTech}{36}
\newcommand{\WM}{37}
\newcommand{\NJU}{38}
\newcommand{\CGNPG}{39}
\newcommand{\NUDT}{40}
\newcommand{\IowaState}{41}
\newcommand{\CQU}{42}
\author{
 F.~P.~An(安丰鹏)$^{\ECUST}$ \and
A.~B.~Balantekin$^{\Wisconsin}$ \and
M.~Bishai$^{\BNL}$ \and
S.~Blyth$^{\NTU}$ \and
G.~F.~Cao(曹国富)$^{\IHEP}$ \and
J.~Cao(曹俊)$^{\IHEP}$ \and
J.~F.~Chang(常劲帆)$^{\IHEP}$ \and
Y.~Chang(张昀)$^{\NUU}$ \and
H.~S.~Chen(陈和生)$^{\IHEP}$ \and
S.~M.~Chen(陈少敏)$^{\TsingHua}$ \and
Y.~Chen(陈羽)$^{\SZU,\ZSU}$ \and
Y.~X.~Chen(陈义学)$^{\NCEPU}$ \and
J.~Cheng(程捷)$^{\IHEP}$ \and
Z.~K.~Cheng(成兆侃)$^{\ZSU}$ \and
J.~J.~Cherwinka$^{\Wisconsin}$ \and
M.~C.~Chu(朱明中)$^{\CUHK}$ \and
J.~P.~Cummings$^{\Siena}$ \and
O.~Dalager$^{\UCI}$ \and
F.~S.~Deng(邓凡水)$^{\USTC}$ \and
Y.~Y.~Ding(丁雅韵)$^{\IHEP}$ \and
M.~V.~Diwan$^{\BNL}$ \and
T.~Dohnal$^{\Charles}$ \and
D.~Dolzhikov$^{\Dubna}$ \and
J.~Dove$^{\UIUC}$ \and
M.~Dvo\v{r}\'{a}k$^{\Charles}$ \and
D.~A.~Dwyer$^{\LBNL}$ \and
J.~P.~Gallo$^{\IIT}$ \and
M.~Gonchar$^{\Dubna}$ \and
G.~H.~Gong(龚光华)$^{\TsingHua}$ \and
H.~Gong(宫辉)$^{\TsingHua}$ \and
M.~Grassi$^{\IHEP,\UCI}$ \and
W.~Q.~Gu(顾文强)$^{\BNL}$ \and
J.~Y.~Guo(郭竞渊)$^{\ZSU}$ \and
L.~Guo(郭磊)$^{\TsingHua}$ \and
X.~H.~Guo(郭新恒)$^{\BNU}$ \and
Y.~H.~Guo(郭宇航)$^{\XJTU}$ \and
Z.~Guo(郭子溢)$^{\TsingHua}$ \and
R.~W.~Hackenburg$^{\BNL}$ \and
S.~Hans$^{\BNL\thanks{Now at: Department of Chemistry and Chemical Technology, Bronx Community College, Bronx, New York  10453}}$ \and
M.~He(何苗)$^{\IHEP}$ \and
K.~M.~Heeger$^{\Yale}$ \and
Y.~K.~Heng(衡月昆)$^{\IHEP}$ \and
%A.~Higuera$^{\UHH}$ \and
Y.~K.~Hor(贺远强)$^{\ZSU}$ \and
Y.~B.~Hsiung(熊怡)$^{\NTU}$ \and
B.~Z.~Hu(胡\CJKfamily{bsmi}貝楨)$^{\NTU}$ \and
J.~R.~Hu(胡健润)$^{\IHEP}$ \and
T.~Hu(胡涛)$^{\IHEP}$ \and
Z.~J.~Hu(胡焯钧)$^{\ZSU}$ \and
H.~X.~Huang(黄翰雄)$^{\CIAE}$ \and
J.~H.~Huang(黄金浩)$^{\IHEP}$ \and
X.~T.~Huang(黄性涛)$^{\SDU}$ \and
Y.~B.~Huang(黄永波)$^{\GXU}$ \and
P.~Huber$^{\VirginiaTech}$ \and
D.~E.~Jaffe$^{\BNL}$ \and
K.~L.~Jen(任\CJKfamily{bsmi}國綸)$^{\NCTU}$ \and
X.~L.~Ji(季筱璐)$^{\IHEP}$ \and
X.~P.~Ji(季向盼)$^{\BNL}$ \and
R.~A.~Johnson$^{\UC}$ \and
D.~Jones$^{\TempleUniversity}$ \and
L.~Kang(康丽)$^{\DGUT}$ \and
S.~H.~Kettell$^{\BNL}$ \and
S.~Kohn$^{\UCB}$ \and
M.~Kramer$^{\LBNL,\UCB}$ \and
T.~J.~Langford$^{\Yale}$ \and
J.~Lee$^{\LBNL}$ \and
J.~H.~C.~Lee(李\CJKfamily{bsmi}曉菁)$^{\HKU}$ \and
R.~T.~Lei(雷瑞霆)$^{\DGUT}$ \and
R.~Leitner$^{\Charles}$ \and
J.~K.~C.~Leung(梁干庄)$^{\HKU}$ \and
F.~Li(李飞)$^{\IHEP}$ \and
H.~L.~Li(李慧玲)$^{\IHEP}$ \and
J.~J.~Li(李进京)$^{\TsingHua}$ \and
Q.~J.~Li(李秋菊)$^{\IHEP}$ \and
R.~H.~Li(李茹慧)$^{\IHEP}$ \and
S.~Li(黎山峰)$^{\DGUT}$ \and
S.~C.~Li$^{\VirginiaTech}$ \and
W.~D.~Li(李卫东)$^{\IHEP}$ \and
X.~N.~Li(李小男)$^{\IHEP}$ \and
X.~Q.~Li(李学潜)$^{\NanKai}$ \and
Y.~F.~Li(李玉峰)$^{\IHEP}$ \and
Z.~B.~Li(李志兵)$^{\ZSU}$ \and
H.~Liang(梁昊)$^{\USTC}$ \and
C.~J.~Lin(林政儒)$^{\LBNL}$ \and
G.~L.~Lin(林贵林)$^{\NCTU}$ \and
S.~Lin(林盛鑫)$^{\DGUT}$ \and
J.~J.~Ling(凌家杰)$^{\ZSU}$ \and
J.~M.~Link$^{\VirginiaTech}$ \and
L.~Littenberg$^{\BNL}$ \and
B.~R.~Littlejohn$^{\IIT}$ \and
J.~C.~Liu(刘金昌)$^{\IHEP}$ \and
J.~L.~Liu(刘江来)$^{\SJTU}$ \and
J.~X.~Liu(刘佳熙)$^{\IHEP}$ \and
C.~Lu(陆昌国)$^{\Princeton}$ \and
H.~Q.~Lu(路浩奇)$^{\IHEP}$ \and
%J.~S.~Lu(陆稼书)$^{\IHEP}$ \and % confirmed by Zeyuan
K.~B.~Luk(陆锦标)$^{\UCB,\LBNL}$ \and
B.~Z.~Ma(马帮争)$^{\SDU}$ \and
X.~B.~Ma(马续波)$^{\NCEPU}$ \and
X.~Y.~Ma(马骁妍)$^{\IHEP}$ \and
Y.~Q.~Ma(马宇倩)$^{\IHEP}$ \and
R.~C.~Mandujano$^{\UCI}$ \and
C.~Marshall$^{\LBNL}$ \and
%D.~A.~Martinez Caicedo$^{\IIT}$ \and % confirmed by Bryce Littlejohn
K.~T.~McDonald$^{\Princeton}$ \and
R.~D.~McKeown$^{\CalTech,\WM}$ \and
Y.~Meng(孟月)$^{\SJTU}$ \and
J.~Napolitano$^{\TempleUniversity}$ \and
D.~Naumov$^{\Dubna}$ \and
E.~Naumova$^{\Dubna}$ \and
T.~M.~T.~Nguyen$^{\NCTU}$ \and
J.~P.~Ochoa-Ricoux$^{\UCI}$ \and
A.~Olshevskiy$^{\Dubna}$ \and
H.-R.~Pan(潘孝儒)$^{\NTU}$ \and
J.~Park$^{\VirginiaTech}$ \and
S.~Patton$^{\LBNL}$ \and
J.~C.~Peng(彭仁杰)$^{\UIUC}$ \and
C.~S.~J.~Pun(潘振声)$^{\HKU}$ \and
F.~Z.~Qi(齐法制)$^{\IHEP}$ \and
M.~Qi(祁鸣)$^{\NJU}$ \and
X.~Qian(钱鑫)$^{\BNL}$ \and
N.~Raper$^{\ZSU}$ \and
J.~Ren(任杰)$^{\CIAE}$ \and
C.~Morales~Reveco$^{\UCI}$ \and
R.~Rosero$^{\BNL}$ \and
B.~Roskovec$^{\UCI}$ \and
X.~C.~Ruan(阮锡超)$^{\CIAE}$ \and
H.~Steiner$^{\UCB,\LBNL}$ \and
J.~L.~Sun(孙吉良)$^{\CGNPG}$ \and
T.~Tmej$^{\Charles}$ \and
K.~Treskov$^{\Dubna}$ \and
W.-H.~Tse(\CJKfamily{bsmi}謝雲皓)$^{\CUHK}$ \and
C.~E.~Tull$^{\LBNL}$ \and
B.~Viren$^{\BNL}$ \and
V.~Vorobel$^{\Charles}$ \and
C.~H.~Wang(王正祥)$^{\NUU}$ \and
J.~Wang(王俊)$^{\ZSU}$ \and
M.~Wang(王萌)$^{\SDU}$ \and
N.~Y.~Wang(王乃彦)$^{\BNU}$ \and
R.~G.~Wang(王瑞光)$^{\IHEP}$ \and
W.~Wang(王为)$^{\ZSU,\WM}$ \and
W.~Wang(王维)$^{\NJU}$ \and
X.~Wang(王玺)$^{\NUDT}$ \and
Y.~Wang(王玉漫)$^{\NJU}$ \and
Y.~F.~Wang(王贻芳)$^{\IHEP}$ \and
Z.~Wang(王铮)$^{\IHEP}$ \and
Z.~Wang(王\hbox{\kern+.2em\scalebox{0.5}[1]{吉}\kern-.1em\scalebox{0.5}[1]{吉}}喆)$^{\TsingHua}$ \and
Z.~M.~Wang(王志民)$^{\IHEP}$ \and
H.~Y.~Wei(魏瀚宇)$^{\BNL}$ \and
L.~H.~Wei(韦良红)$^{\IHEP}$ \and
L.~J.~Wen(温良剑)$^{\IHEP}$ \and
K.~Whisnant$^{\IowaState}$ \and
C.~G.~White$^{\IIT}$ \and
H.~L.~H.~Wong(黄显诺)$^{\UCB,\LBNL}$ \and
E.~Worcester$^{\BNL}$ \and
D.~R.~Wu(吴帝儒)$^{\IHEP}$ \and
F.~L.~Wu(武方亮)$^{\NJU}$ \and
Q.~Wu(吴群)$^{\SDU}$ \and
W.~J.~Wu(吴文杰)$^{\IHEP}$ \and
D.~M.~Xia(夏冬梅)$^{\CQU}$ \and
Z.~Q.~Xie(谢章权)$^{\IHEP}$ \and
Z.~Z.~Xing(邢志忠)$^{\IHEP}$ \and
H.~K.~Xu(许杭锟)$^{\IHEP}$ \and
J.~L.~Xu(徐吉磊)$^{\IHEP}$ \and
T.~Xu(徐彤)$^{\TsingHua}$ \and
T.~Xue(薛涛)$^{\TsingHua}$ \and
C.~G.~Yang(杨长根)$^{\IHEP}$ \and
L.~Yang(杨雷)$^{\DGUT}$ \and
Y.~Z.~Yang(杨玉梓)$^{\TsingHua}$ \and
H.~F.~Yao(姚海峰)$^{\IHEP}$ \and
M.~Ye(叶梅)$^{\IHEP}$ \and
M.~Yeh(叶铭芳)$^{\BNL}$ \and
B.~L.~Young(杨炳麟)$^{\IowaState}$ \and
H.~Z.~Yu(余泓钊)$^{\ZSU}$ \and
Z.~Y.~Yu(于泽源)$^{\IHEP}$ \and
B.~B.~Yue(岳保彪)$^{\ZSU}$ \and
V.~Zavadskyi$^{\Dubna}$ \and %Zavadskyi confirmed he is not from BNL, previously BNL and Dubna are both there
S.~Zeng(曾珊)$^{\IHEP}$ \and
Y.~Zeng(曾裕达)$^{\ZSU}$ \and
L.~Zhan(占亮)$^{\IHEP}$ \and
C.~Zhang(张超)$^{\BNL}$ \and
F.~Y.~Zhang(张飞洋)$^{\SJTU}$ \and
H.~H.~Zhang(张宏浩)$^{\ZSU}$ \and
J.~W.~Zhang(张家文)$^{\IHEP}$ \and
Q.~M.~Zhang(张清民)$^{\XJTU}$ \and
S.~Q.~Zhang(张石其)$^{\ZSU}$ \and
X.~T.~Zhang(张玄同)$^{\IHEP}$ \and
Y.~M.~Zhang(张玉美)$^{\ZSU}$ \and
Y.~X.~Zhang(张一心)$^{\CGNPG}$ \and
Y.~Y.~Zhang(张园园)$^{\SJTU}$ \and
Z.~J.~Zhang(张志坚)$^{\DGUT}$ \and
Z.~P.~Zhang(张子平)$^{\USTC}$ \and
Z.~Y.~Zhang(张智勇)$^{\IHEP}$ \and
J.~Zhao(赵洁)$^{\IHEP}$ \and
R.~Z.~Zhao(赵润泽)$^{\IHEP}$ \and
L.~Zhou(周莉)$^{\IHEP}$ \and
H.~L.~Zhuang(庄红林)$^{\IHEP}$ \and
J.~H.~Zou(邹佳恒)$^{\IHEP}$ \and
}

\maketitle %%%%%%%% NOTE THAT maketitle COMMAND APPEARS IN THE AUTHOR LIST %%%%%%%   

\address{
\vspace{0.3cm}
{\normalsize (Daya Bay Collaboration)} \\ 
\vspace{0.3cm}
$^{\ECUST}$Institute of Modern Physics, East China University of Science and Technology, Shanghai \\ 
$^{\Wisconsin}$University~of~Wisconsin, Madison, Wisconsin 53706 \\ 
$^{\BNL}$Brookhaven~National~Laboratory, Upton, New York 11973 \\ 
$^{\NTU}$Department of Physics, National~Taiwan~University, Taipei \\ 
$^{\IHEP}$Institute~of~High~Energy~Physics, Beijing \\ 
$^{\NUU}$National~United~University, Miao-Li \\ 
$^{\TsingHua}$Department~of~Engineering~Physics, Tsinghua~University, Beijing \\ 
$^{\SZU}$Shenzhen~University, Shenzhen \\ 
$^{\ZSU}$Sun Yat-Sen (Zhongshan) University, Guangzhou \\ 
$^{\NCEPU}$North~China~Electric~Power~University, Beijing \\ 
$^{\CUHK}$Chinese~University~of~Hong~Kong, Hong~Kong \\ 
$^{\Siena}$Siena~College, Loudonville, New York  12211 \\ 
$^{\UCI}$Department of Physics and Astronomy, University of California, Irvine, California 92697 \\ 
$^{\USTC}$University~of~Science~and~Technology~of~China, Hefei \\ 
$^{\Charles}$Charles~University, Faculty~of~Mathematics~and~Physics, Prague \\ 
$^{\Dubna}$Joint~Institute~for~Nuclear~Research, Dubna, Moscow~Region \\ 
$^{\UIUC}$Department of Physics, University~of~Illinois~at~Urbana-Champaign, Urbana, Illinois 61801 \\ 
$^{\LBNL}$Lawrence~Berkeley~National~Laboratory, Berkeley, California 94720 \\ 
$^{\IIT}$Department of Physics, Illinois~Institute~of~Technology, Chicago, Illinois  60616 \\ 
$^{\BNU}$Beijing~Normal~University, Beijing \\ 
$^{\XJTU}$Department of Nuclear Science and Technology, School of Energy and Power Engineering, Xi'an Jiaotong University, Xi'an \\ 
$^{\Yale}$Wright~Laboratory and Department~of~Physics, Yale~University, New~Haven, Connecticut 06520 \\ 
$^{\CIAE}$China~Institute~of~Atomic~Energy, Beijing \\ 
$^{\SDU}$Shandong~University, Jinan \\ 
$^{\GXU}$Guangxi University, No.100 Daxue East Road, Nanning \\ 
$^{\VirginiaTech}$Center for Neutrino Physics, Virginia~Tech, Blacksburg, Virginia  24061 \\ 
$^{\NCTU}$Institute~of~Physics, National~Chiao-Tung~University, Hsinchu \\ 
$^{\UC}$Department of Physics, University~of~Cincinnati, Cincinnati, Ohio 45221 \\ 
$^{\TempleUniversity}$Department~of~Physics, College~of~Science~and~Technology, Temple~University, Philadelphia, Pennsylvania  19122 \\ 
$^{\DGUT}$Dongguan~University~of~Technology, Dongguan \\ 
$^{\UCB}$Department of Physics, University~of~California, Berkeley, California  94720 \\ 
$^{\HKU}$Department of Physics, The~University~of~Hong~Kong, Pokfulam, Hong~Kong \\ 
$^{\NanKai}$School of Physics, Nankai~University, Tianjin \\ 
$^{\SJTU}$Department of Physics and Astronomy, Shanghai Jiao Tong University, Shanghai Laboratory for Particle Physics and Cosmology, Shanghai \\ 
$^{\Princeton}$Joseph Henry Laboratories, Princeton~University, Princeton, New~Jersey 08544 \\ 
$^{\CalTech}$California~Institute~of~Technology, Pasadena, California 91125 \\ 
$^{\WM}$College~of~William~and~Mary, Williamsburg, Virginia  23187 \\ 
$^{\NJU}$Nanjing~University, Nanjing \\ 
$^{\CGNPG}$China General Nuclear Power Group, Shenzhen \\ 
$^{\NUDT}$College of Electronic Science and Engineering, National University of Defense Technology, Changsha \\ 
$^{\IowaState}$Iowa~State~University, Ames, Iowa  50011 \\ 
$^{\CQU}$Chongqing University, Chongqing \\ 
} 


==> Antineutrino Energy Spectrum Unfolding Based on the Daya Bay Measurement and Its Application/DayaBayCollaboration.tex <==
%%% Generation information for this file
%%% Wed Apr  3 08:26:54 2019
%%% /Users/djaffe/Documents/Reactor/work/trunk/NuWa-trunk/dybgaudi/Documentation/AuthorList/2019_ReactorDecomposition
%%% ../AuthGen.py dyb_collabotion_20180427.xls 20180427 
\newcommand{\ECUST}{\affiliation{Institute of Modern Physics, East China University of Science and Technology, Shanghai}}
\newcommand{\IHEP}{\affiliation{Institute~of~High~Energy~Physics, Beijing}}
\newcommand{\Wisconsin}{\affiliation{University~of~Wisconsin, Madison, Wisconsin 53706}}
\newcommand{\Yale}{\affiliation{Wright~Laboratory and Department~of~Physics, Yale~University, New~Haven, Connecticut 06520}} %%%% 20170227 add Wright Lab
\newcommand{\BNL}{\affiliation{Brookhaven~National~Laboratory, Upton, New York 11973}}
\newcommand{\NTU}{\affiliation{Department of Physics, National~Taiwan~University, Taipei}}
\newcommand{\NUU}{\affiliation{National~United~University, Miao-Li}}
\newcommand{\Dubna}{\affiliation{Joint~Institute~for~Nuclear~Research, Dubna, Moscow~Region}}
\newcommand{\CalTech}{\affiliation{California~Institute~of~Technology, Pasadena, California 91125}}
\newcommand{\CUHK}{\affiliation{Chinese~University~of~Hong~Kong, Hong~Kong}}
\newcommand{\NCTU}{\affiliation{Institute~of~Physics, National~Chiao-Tung~University, Hsinchu}}
\newcommand{\NJU}{\affiliation{Nanjing~University, Nanjing}}
\newcommand{\TsingHua}{\affiliation{Department~of~Engineering~Physics, Tsinghua~University, Beijing}}
\newcommand{\SZU}{\affiliation{Shenzhen~University, Shenzhen}}
\newcommand{\NCEPU}{\affiliation{North~China~Electric~Power~University, Beijing}}
\newcommand{\Siena}{\affiliation{Siena~College, Loudonville, New York  12211}}
\newcommand{\IIT}{\affiliation{Department of Physics, Illinois~Institute~of~Technology, Chicago, Illinois  60616}}
\newcommand{\LBNL}{\affiliation{Lawrence~Berkeley~National~Laboratory, Berkeley, California 94720}}
\newcommand{\UIUC}{\affiliation{Department of Physics, University~of~Illinois~at~Urbana-Champaign, Urbana, Illinois 61801}}
\newcommand{\SJTU}{\affiliation{Department of Physics and Astronomy, Shanghai Jiao Tong University, Shanghai Laboratory for Particle Physics and Cosmology, Shanghai}}
\newcommand{\BNU}{\affiliation{Beijing~Normal~University, Beijing}}
\newcommand{\WM}{\affiliation{College~of~William~and~Mary, Williamsburg, Virginia  23187}}
\newcommand{\Princeton}{\affiliation{Joseph Henry Laboratories, Princeton~University, Princeton, New~Jersey 08544}}
\newcommand{\VirginiaTech}{\affiliation{Center for Neutrino Physics, Virginia~Tech, Blacksburg, Virginia  24061}}
\newcommand{\CIAE}{\affiliation{China~Institute~of~Atomic~Energy, Beijing}}
\newcommand{\SDU}{\affiliation{Shandong~University, Jinan}}
\newcommand{\NanKai}{\affiliation{School of Physics, Nankai~University, Tianjin}}
\newcommand{\UC}{\affiliation{Department of Physics, University~of~Cincinnati, Cincinnati, Ohio 45221}}
\newcommand{\DGUT}{\affiliation{Dongguan~University~of~Technology, Dongguan}}
\newcommand{\XJTU}{\affiliation{Department of Nuclear Science and Technology, School of Energy and Power Engineering, Xi'an Jiaotong University, Xi'an}}%%updated 20161215 {Xi'an Jiaotong University, Xi'an}}
\newcommand{\UCB}{\affiliation{Department of Physics, University~of~California, Berkeley, California  94720}}
\newcommand{\HKU}{\affiliation{Department of Physics, The~University~of~Hong~Kong, Pokfulam, Hong~Kong}}
\newcommand{\UH}{\affiliation{Department of Physics, University~of~Houston, Houston, Texas  77204}}
\newcommand{\Charles}{\affiliation{Charles~University, Faculty~of~Mathematics~and~Physics, Prague}} %updated20140819
\newcommand{\USTC}{\affiliation{University~of~Science~and~Technology~of~China, Hefei}}
\newcommand{\TempleUniversity}{\affiliation{Department~of~Physics, College~of~Science~and~Technology, Temple~University, Philadelphia, Pennsylvania  19122}}
\newcommand{\CUC}{\affiliation{Instituto de F\'isica, Pontificia Universidad Cat\'olica de Chile, Santiago}} % update 20140911 use r23215 for Spanish
\newcommand{\CGNPG}{\affiliation{China General Nuclear Power Group, Shenzhen}}% update 20170729 add city. updated 20140724 China~Guangdong~Nuclear~Power~Group, Shenzhen}}
\newcommand{\NUDT}{\affiliation{College of Electronic Science and Engineering, National University of Defense Technology, Changsha}} % added 20140111
\newcommand{\IowaState}{\affiliation{Iowa~State~University, Ames, Iowa  50011}}
\newcommand{\ZSU}{\affiliation{Sun Yat-Sen (Zhongshan) University, Guangzhou}}
\newcommand{\CQU}{\affiliation{Chongqing University, Chongqing}} % add 20150417
\newcommand{\BCC}{\altaffiliation[Now at ]{Department of Chemistry and Chemical Technology, Bronx Community College, Bronx, New York  10453}} % add 20160311 for Sunej's 'now at'

\newcommand{\UCI}{\affiliation{Department of Physics and Astronomy, University of California, Irvine, California 92697}} %20190209 for Pedro's new digs
\author{D.~Adey}\IHEP
\author{F.~P.~An}\ECUST
\author{A.~B.~Balantekin}\Wisconsin
\author{H.~R.~Band}\Yale
\author{M.~Bishai}\BNL
\author{S.~Blyth}\NTU
\author{D.~Cao}\NJU
\author{G.~F.~Cao}\IHEP
\author{J.~Cao}\IHEP
\author{J.~F.~Chang}\IHEP
\author{Y.~Chang}\NUU
\author{H.~S.~Chen}\IHEP
\author{S.~M.~Chen}\TsingHua
\author{Y.~Chen}\SZU\ZSU
\author{Y.~X.~Chen}\NCEPU
\author{J.~Cheng}\IHEP
\author{Z.~K.~Cheng}\ZSU
\author{J.~J.~Cherwinka}\Wisconsin
\author{M.~C.~Chu}\CUHK
\author{A.~Chukanov}\Dubna
\author{J.~P.~Cummings}\Siena
\author{N.~Dash}\IHEP
\author{F.~S.~Deng}\USTC
\author{Y.~Y.~Ding}\IHEP
\author{M.~V.~Diwan}\BNL
\author{T.~Dohnal}\Charles
\author{J.~Dove}\UIUC
\author{M.~Dvo\v{r}\'{a}k}\Charles
\author{D.~A.~Dwyer}\LBNL
\author{M.~Gonchar}\Dubna
\author{G.~H.~Gong}\TsingHua
\author{H.~Gong}\TsingHua
\author{W.~Q.~Gu}\BNL
\author{J.~Y.~Guo}\ZSU
\author{L.~Guo}\TsingHua
\author{X.~H.~Guo}\BNU
\author{Y.~H.~Guo}\XJTU
\author{Z.~Guo}\TsingHua
\author{R.~W.~Hackenburg}\BNL
\author{S.~Hans}\BCC\BNL
\author{M.~He}\IHEP
\author{K.~M.~Heeger}\Yale
\author{Y.~K.~Heng}\IHEP
\author{A.~Higuera}\UH
\author{Y.~K.~Hor}\ZSU
\author{Y.~B.~Hsiung}\NTU
\author{B.~Z.~Hu}\NTU
\author{J.~R.~Hu}\IHEP
\author{T.~Hu}\IHEP
\author{Z.~J.~Hu}\ZSU
\author{H.~X.~Huang}\CIAE
\author{X.~T.~Huang}\SDU
\author{Y.~B.~Huang}\IHEP
\author{P.~Huber}\VirginiaTech
\author{D.~E.~Jaffe}\BNL
\author{K.~L.~Jen}\NCTU
\author{X.~L.~Ji}\IHEP
\author{X.~P.~Ji}\BNL
\author{R.~A.~Johnson}\UC
\author{D.~Jones}\TempleUniversity
\author{L.~Kang}\DGUT
\author{S.~H.~Kettell}\BNL
\author{L.~W.~Koerner}\UH
\author{S.~Kohn}\UCB
\author{M.~Kramer}\LBNL\UCB
\author{T.~J.~Langford}\Yale
\author{J.~Lee}\LBNL
\author{J.~H.~C.~Lee}\HKU
\author{R.~T.~Lei}\DGUT
\author{R.~Leitner}\Charles
\author{J.~K.~C.~Leung}\HKU
\author{C.~Li}\SDU
\author{F.~Li}\IHEP
\author{H.~L.~Li}\IHEP
\author{Q.~J.~Li}\IHEP
\author{S.~Li}\DGUT
\author{S.~C.~Li}\VirginiaTech
\author{S.~J.~Li}\ZSU
\author{W.~D.~Li}\IHEP
\author{X.~N.~Li}\IHEP
\author{X.~Q.~Li}\NanKai
\author{Y.~F.~Li}\IHEP
\author{Z.~B.~Li}\ZSU
\author{H.~Liang}\USTC
\author{C.~J.~Lin}\LBNL
\author{G.~L.~Lin}\NCTU
\author{S.~Lin}\DGUT
\author{J.~J.~Ling}\ZSU
\author{J.~M.~Link}\VirginiaTech
\author{L.~Littenberg}\BNL
\author{B.~R.~Littlejohn}\IIT
\author{J.~C.~Liu}\IHEP
\author{J.~L.~Liu}\SJTU
\author{Y.~Liu}\SDU
\author{Y.~H.~Liu}\NJU
\author{C.~Lu}\Princeton
\author{H.~Q.~Lu}\IHEP
\author{J.~S.~Lu}\IHEP
\author{K.~B.~Luk}\UCB\LBNL
\author{X.~B.~Ma}\NCEPU
\author{X.~Y.~Ma}\IHEP
\author{Y.~Q.~Ma}\IHEP
\author{C.~Marshall}\LBNL
\author{D.~A.~Martinez Caicedo}\IIT
\author{K.~T.~McDonald}\Princeton
\author{R.~D.~McKeown}\CalTech\WM
\author{I.~Mitchell}\UH
\author{L.~Mora Lepin}\CUC
\author{J.~Napolitano}\TempleUniversity
\author{D.~Naumov}\Dubna
\author{E.~Naumova}\Dubna
\author{J.~P.~Ochoa-Ricoux}\CUC\UCI
\author{A.~Olshevskiy}\Dubna
\author{H.-R.~Pan}\NTU
\author{J.~Park}\VirginiaTech
\author{S.~Patton}\LBNL
\author{V.~Pec}\Charles
\author{J.~C.~Peng}\UIUC
\author{L.~Pinsky}\UH
\author{C.~S.~J.~Pun}\HKU
\author{F.~Z.~Qi}\IHEP
\author{M.~Qi}\NJU
\author{X.~Qian}\BNL
\author{N.~Raper}\ZSU
\author{J.~Ren}\CIAE
\author{R.~Rosero}\BNL
\author{B.~Roskovec}\UCI
\author{X.~C.~Ruan}\CIAE
\author{H.~Steiner}\UCB\LBNL
\author{J.~L.~Sun}\CGNPG
\author{K.~Treskov}\Dubna
\author{W.-H.~Tse}\CUHK
\author{C.~E.~Tull}\LBNL
\author{B.~Viren}\BNL
\author{V.~Vorobel}\Charles
\author{C.~H.~Wang}\NUU
\author{J.~Wang}\ZSU
\author{M.~Wang}\SDU
\author{N.~Y.~Wang}\BNU
\author{R.~G.~Wang}\IHEP
\author{W.~Wang}\ZSU\WM
\author{W.~Wang}\NJU
\author{X.~Wang}\NUDT
\author{Y.~Wang}\NJU
\author{Y.~F.~Wang}\IHEP
\author{Z.~Wang}\IHEP
\author{Z.~Wang}\TsingHua
\author{Z.~M.~Wang}\IHEP
\author{H.~Y.~Wei}\BNL
\author{L.~H.~Wei}\IHEP
\author{L.~J.~Wen}\IHEP
\author{K.~Whisnant}\IowaState
\author{C.~G.~White}\IIT
\author{H.~L.~H.~Wong}\UCB\LBNL
\author{S.~C.~F.~Wong}\ZSU
\author{E.~Worcester}\BNL
\author{Q.~Wu}\SDU
\author{W.~J.~Wu}\IHEP
\author{D.~M.~Xia}\CQU
\author{Z.~Z.~Xing}\IHEP
\author{J.~L.~Xu}\IHEP
\author{T.~Xue}\TsingHua
\author{C.~G.~Yang}\IHEP
\author{L.~Yang}\DGUT
\author{M.~S.~Yang}\IHEP
\author{Y.~Z.~Yang}\TsingHua
\author{M.~Ye}\IHEP
\author{M.~Yeh}\BNL
\author{B.~L.~Young}\IowaState
\author{H.~Z.~Yu}\ZSU
\author{Z.~Y.~Yu}\IHEP
\author{B.~B.~Yue}\ZSU
\author{S.~Zeng}\IHEP
\author{Y.~Zeng}\ZSU
\author{L.~Zhan}\IHEP
\author{C.~Zhang}\BNL
\author{C.~C.~Zhang}\IHEP
\author{F.~Y.~Zhang}\SJTU
\author{H.~H.~Zhang}\ZSU
\author{J.~W.~Zhang}\IHEP
\author{Q.~M.~Zhang}\XJTU
\author{R.~Zhang}\NJU
\author{X.~F.~Zhang}\IHEP
\author{X.~T.~Zhang}\IHEP
\author{Y.~M.~Zhang}\ZSU
\author{Y.~M.~Zhang}\TsingHua
\author{Y.~X.~Zhang}\CGNPG
\author{Y.~Y.~Zhang}\SJTU
\author{Z.~J.~Zhang}\DGUT
\author{Z.~P.~Zhang}\USTC
\author{Z.~Y.~Zhang}\IHEP
\author{J.~Zhao}\IHEP
\author{L.~Zhou}\IHEP
\author{H.~L.~Zhuang}\IHEP
\author{J.~H.~Zou}\IHEP



==> DayaBayCollaboration.tex <==
%%% Generation information for this file
%%% Wed Apr  3 08:26:54 2019
%%% /Users/djaffe/Documents/Reactor/work/trunk/NuWa-trunk/dybgaudi/Documentation/AuthorList/2019_ReactorDecomposition
%%% ../AuthGen.py dyb_collabotion_20180427.xls 20180427 
\newcommand{\ECUST}{\affiliation{Institute of Modern Physics, East China University of Science and Technology, Shanghai}}
\newcommand{\IHEP}{\affiliation{Institute~of~High~Energy~Physics, Beijing}}
\newcommand{\Wisconsin}{\affiliation{University~of~Wisconsin, Madison, Wisconsin 53706}}
\newcommand{\Yale}{\affiliation{Wright~Laboratory and Department~of~Physics, Yale~University, New~Haven, Connecticut 06520}} %%%% 20170227 add Wright Lab
\newcommand{\BNL}{\affiliation{Brookhaven~National~Laboratory, Upton, New York 11973}}
\newcommand{\NTU}{\affiliation{Department of Physics, National~Taiwan~University, Taipei}}
\newcommand{\NUU}{\affiliation{National~United~University, Miao-Li}}
\newcommand{\Dubna}{\affiliation{Joint~Institute~for~Nuclear~Research, Dubna, Moscow~Region}}
\newcommand{\CalTech}{\affiliation{California~Institute~of~Technology, Pasadena, California 91125}}
\newcommand{\CUHK}{\affiliation{Chinese~University~of~Hong~Kong, Hong~Kong}}
\newcommand{\NCTU}{\affiliation{Institute~of~Physics, National~Chiao-Tung~University, Hsinchu}}
\newcommand{\NJU}{\affiliation{Nanjing~University, Nanjing}}
\newcommand{\TsingHua}{\affiliation{Department~of~Engineering~Physics, Tsinghua~University, Beijing}}
\newcommand{\SZU}{\affiliation{Shenzhen~University, Shenzhen}}
\newcommand{\NCEPU}{\affiliation{North~China~Electric~Power~University, Beijing}}
\newcommand{\Siena}{\affiliation{Siena~College, Loudonville, New York  12211}}
\newcommand{\IIT}{\affiliation{Department of Physics, Illinois~Institute~of~Technology, Chicago, Illinois  60616}}
\newcommand{\LBNL}{\affiliation{Lawrence~Berkeley~National~Laboratory, Berkeley, California 94720}}
\newcommand{\UIUC}{\affiliation{Department of Physics, University~of~Illinois~at~Urbana-Champaign, Urbana, Illinois 61801}}
\newcommand{\SJTU}{\affiliation{Department of Physics and Astronomy, Shanghai Jiao Tong University, Shanghai Laboratory for Particle Physics and Cosmology, Shanghai}}
\newcommand{\BNU}{\affiliation{Beijing~Normal~University, Beijing}}
\newcommand{\WM}{\affiliation{College~of~William~and~Mary, Williamsburg, Virginia  23187}}
\newcommand{\Princeton}{\affiliation{Joseph Henry Laboratories, Princeton~University, Princeton, New~Jersey 08544}}
\newcommand{\VirginiaTech}{\affiliation{Center for Neutrino Physics, Virginia~Tech, Blacksburg, Virginia  24061}}
\newcommand{\CIAE}{\affiliation{China~Institute~of~Atomic~Energy, Beijing}}
\newcommand{\SDU}{\affiliation{Shandong~University, Jinan}}
\newcommand{\NanKai}{\affiliation{School of Physics, Nankai~University, Tianjin}}
\newcommand{\UC}{\affiliation{Department of Physics, University~of~Cincinnati, Cincinnati, Ohio 45221}}
\newcommand{\DGUT}{\affiliation{Dongguan~University~of~Technology, Dongguan}}
\newcommand{\XJTU}{\affiliation{Department of Nuclear Science and Technology, School of Energy and Power Engineering, Xi'an Jiaotong University, Xi'an}}%%updated 20161215 {Xi'an Jiaotong University, Xi'an}}
\newcommand{\UCB}{\affiliation{Department of Physics, University~of~California, Berkeley, California  94720}}
\newcommand{\HKU}{\affiliation{Department of Physics, The~University~of~Hong~Kong, Pokfulam, Hong~Kong}}
\newcommand{\UH}{\affiliation{Department of Physics, University~of~Houston, Houston, Texas  77204}}
\newcommand{\Charles}{\affiliation{Charles~University, Faculty~of~Mathematics~and~Physics, Prague}} %updated20140819
\newcommand{\USTC}{\affiliation{University~of~Science~and~Technology~of~China, Hefei}}
\newcommand{\TempleUniversity}{\affiliation{Department~of~Physics, College~of~Science~and~Technology, Temple~University, Philadelphia, Pennsylvania  19122}}
\newcommand{\CUC}{\affiliation{Instituto de F\'isica, Pontificia Universidad Cat\'olica de Chile, Santiago}} % update 20140911 use r23215 for Spanish
\newcommand{\CGNPG}{\affiliation{China General Nuclear Power Group, Shenzhen}}% update 20170729 add city. updated 20140724 China~Guangdong~Nuclear~Power~Group, Shenzhen}}
\newcommand{\NUDT}{\affiliation{College of Electronic Science and Engineering, National University of Defense Technology, Changsha}} % added 20140111
\newcommand{\IowaState}{\affiliation{Iowa~State~University, Ames, Iowa  50011}}
\newcommand{\ZSU}{\affiliation{Sun Yat-Sen (Zhongshan) University, Guangzhou}}
\newcommand{\CQU}{\affiliation{Chongqing University, Chongqing}} % add 20150417
\newcommand{\BCC}{\altaffiliation[Now at ]{Department of Chemistry and Chemical Technology, Bronx Community College, Bronx, New York  10453}} % add 20160311 for Sunej's 'now at'

\newcommand{\UCI}{\affiliation{Department of Physics and Astronomy, University of California, Irvine, California 92697}} %20190209 for Pedro's new digs
\author{D.~Adey}\IHEP
\author{F.~P.~An}\ECUST
\author{A.~B.~Balantekin}\Wisconsin
\author{H.~R.~Band}\Yale
\author{M.~Bishai}\BNL
\author{S.~Blyth}\NTU
\author{D.~Cao}\NJU
\author{G.~F.~Cao}\IHEP
\author{J.~Cao}\IHEP
\author{J.~F.~Chang}\IHEP
\author{Y.~Chang}\NUU
\author{H.~S.~Chen}\IHEP
\author{S.~M.~Chen}\TsingHua
\author{Y.~Chen}\SZU\ZSU
\author{Y.~X.~Chen}\NCEPU
\author{J.~Cheng}\IHEP
\author{Z.~K.~Cheng}\ZSU
\author{J.~J.~Cherwinka}\Wisconsin
\author{M.~C.~Chu}\CUHK
\author{A.~Chukanov}\Dubna
\author{J.~P.~Cummings}\Siena
\author{N.~Dash}\IHEP
\author{F.~S.~Deng}\USTC
\author{Y.~Y.~Ding}\IHEP
\author{M.~V.~Diwan}\BNL
\author{T.~Dohnal}\Charles
\author{J.~Dove}\UIUC
\author{M.~Dvo\v{r}\'{a}k}\Charles
\author{D.~A.~Dwyer}\LBNL
\author{M.~Gonchar}\Dubna
\author{G.~H.~Gong}\TsingHua
\author{H.~Gong}\TsingHua
\author{W.~Q.~Gu}\BNL
\author{J.~Y.~Guo}\ZSU
\author{L.~Guo}\TsingHua
\author{X.~H.~Guo}\BNU
\author{Y.~H.~Guo}\XJTU
\author{Z.~Guo}\TsingHua
\author{R.~W.~Hackenburg}\BNL
\author{S.~Hans}\BCC\BNL
\author{M.~He}\IHEP
\author{K.~M.~Heeger}\Yale
\author{Y.~K.~Heng}\IHEP
\author{A.~Higuera}\UH
\author{Y.~K.~Hor}\ZSU
\author{Y.~B.~Hsiung}\NTU
\author{B.~Z.~Hu}\NTU
\author{J.~R.~Hu}\IHEP
\author{T.~Hu}\IHEP
\author{Z.~J.~Hu}\ZSU
\author{H.~X.~Huang}\CIAE
\author{X.~T.~Huang}\SDU
\author{Y.~B.~Huang}\IHEP
\author{P.~Huber}\VirginiaTech
\author{D.~E.~Jaffe}\BNL
\author{K.~L.~Jen}\NCTU
\author{X.~L.~Ji}\IHEP
\author{X.~P.~Ji}\BNL
\author{R.~A.~Johnson}\UC
\author{D.~Jones}\TempleUniversity
\author{L.~Kang}\DGUT
\author{S.~H.~Kettell}\BNL
\author{L.~W.~Koerner}\UH
\author{S.~Kohn}\UCB
\author{M.~Kramer}\LBNL\UCB
\author{T.~J.~Langford}\Yale
\author{J.~Lee}\LBNL
\author{J.~H.~C.~Lee}\HKU
\author{R.~T.~Lei}\DGUT
\author{R.~Leitner}\Charles
\author{J.~K.~C.~Leung}\HKU
\author{C.~Li}\SDU
\author{F.~Li}\IHEP
\author{H.~L.~Li}\IHEP
\author{Q.~J.~Li}\IHEP
\author{S.~Li}\DGUT
\author{S.~C.~Li}\VirginiaTech
\author{S.~J.~Li}\ZSU
\author{W.~D.~Li}\IHEP
\author{X.~N.~Li}\IHEP
\author{X.~Q.~Li}\NanKai
\author{Y.~F.~Li}\IHEP
\author{Z.~B.~Li}\ZSU
\author{H.~Liang}\USTC
\author{C.~J.~Lin}\LBNL
\author{G.~L.~Lin}\NCTU
\author{S.~Lin}\DGUT
\author{J.~J.~Ling}\ZSU
\author{J.~M.~Link}\VirginiaTech
\author{L.~Littenberg}\BNL
\author{B.~R.~Littlejohn}\IIT
\author{J.~C.~Liu}\IHEP
\author{J.~L.~Liu}\SJTU
\author{Y.~Liu}\SDU
\author{Y.~H.~Liu}\NJU
\author{C.~Lu}\Princeton
\author{H.~Q.~Lu}\IHEP
\author{J.~S.~Lu}\IHEP
\author{K.~B.~Luk}\UCB\LBNL
\author{X.~B.~Ma}\NCEPU
\author{X.~Y.~Ma}\IHEP
\author{Y.~Q.~Ma}\IHEP
\author{C.~Marshall}\LBNL
\author{D.~A.~Martinez Caicedo}\IIT
\author{K.~T.~McDonald}\Princeton
\author{R.~D.~McKeown}\CalTech\WM
\author{I.~Mitchell}\UH
\author{L.~Mora Lepin}\CUC
\author{J.~Napolitano}\TempleUniversity
\author{D.~Naumov}\Dubna
\author{E.~Naumova}\Dubna
\author{J.~P.~Ochoa-Ricoux}\CUC\UCI
\author{A.~Olshevskiy}\Dubna
\author{H.-R.~Pan}\NTU
\author{J.~Park}\VirginiaTech
\author{S.~Patton}\LBNL
\author{V.~Pec}\Charles
\author{J.~C.~Peng}\UIUC
\author{L.~Pinsky}\UH
\author{C.~S.~J.~Pun}\HKU
\author{F.~Z.~Qi}\IHEP
\author{M.~Qi}\NJU
\author{X.~Qian}\BNL
\author{N.~Raper}\ZSU
\author{J.~Ren}\CIAE
\author{R.~Rosero}\BNL
\author{B.~Roskovec}\UCI
\author{X.~C.~Ruan}\CIAE
\author{H.~Steiner}\UCB\LBNL
\author{J.~L.~Sun}\CGNPG
\author{K.~Treskov}\Dubna
\author{W.-H.~Tse}\CUHK
\author{C.~E.~Tull}\LBNL
\author{B.~Viren}\BNL
\author{V.~Vorobel}\Charles
\author{C.~H.~Wang}\NUU
\author{J.~Wang}\ZSU
\author{M.~Wang}\SDU
\author{N.~Y.~Wang}\BNU
\author{R.~G.~Wang}\IHEP
\author{W.~Wang}\ZSU\WM
\author{W.~Wang}\NJU
\author{X.~Wang}\NUDT
\author{Y.~Wang}\NJU
\author{Y.~F.~Wang}\IHEP
\author{Z.~Wang}\IHEP
\author{Z.~Wang}\TsingHua
\author{Z.~M.~Wang}\IHEP
\author{H.~Y.~Wei}\BNL
\author{L.~H.~Wei}\IHEP
\author{L.~J.~Wen}\IHEP
\author{K.~Whisnant}\IowaState
\author{C.~G.~White}\IIT
\author{H.~L.~H.~Wong}\UCB\LBNL
\author{S.~C.~F.~Wong}\ZSU
\author{E.~Worcester}\BNL
\author{Q.~Wu}\SDU
\author{W.~J.~Wu}\IHEP
\author{D.~M.~Xia}\CQU
\author{Z.~Z.~Xing}\IHEP
\author{J.~L.~Xu}\IHEP
\author{T.~Xue}\TsingHua
\author{C.~G.~Yang}\IHEP
\author{L.~Yang}\DGUT
\author{M.~S.~Yang}\IHEP
\author{Y.~Z.~Yang}\TsingHua
\author{M.~Ye}\IHEP
\author{M.~Yeh}\BNL
\author{B.~L.~Young}\IowaState
\author{H.~Z.~Yu}\ZSU
\author{Z.~Y.~Yu}\IHEP
\author{B.~B.~Yue}\ZSU
\author{S.~Zeng}\IHEP
\author{Y.~Zeng}\ZSU
\author{L.~Zhan}\IHEP
\author{C.~Zhang}\BNL
\author{C.~C.~Zhang}\IHEP
\author{F.~Y.~Zhang}\SJTU
\author{H.~H.~Zhang}\ZSU
\author{J.~W.~Zhang}\IHEP
\author{Q.~M.~Zhang}\XJTU
\author{R.~Zhang}\NJU
\author{X.~F.~Zhang}\IHEP
\author{X.~T.~Zhang}\IHEP
\author{Y.~M.~Zhang}\ZSU
\author{Y.~M.~Zhang}\TsingHua
\author{Y.~X.~Zhang}\CGNPG
\author{Y.~Y.~Zhang}\SJTU
\author{Z.~J.~Zhang}\DGUT
\author{Z.~P.~Zhang}\USTC
\author{Z.~Y.~Zhang}\IHEP
\author{J.~Zhao}\IHEP
\author{L.~Zhou}\IHEP
\author{H.~L.~Zhuang}\IHEP
\author{J.~H.~Zou}\IHEP


